Self-Supervised Intrinsic Image Decomposition

Intrinsic decomposition from a single image is a highly challenging task, due to its inherent ambiguity and the scarcity of training data. In contrast to traditional fully supervised learning approaches, in this paper we propose learning intrinsic image decomposition by explaining the input image. Our model, the Rendered Intrinsics Network (RIN), joins together an image decomposition pipeline, which predicts reflectance, shape, and lighting conditions given a single image, with a recombination function, a learned shading model used to recompose the original input based off of intrinsic image predictions. Our network can then use unsupervised reconstruction error as an additional signal to improve its intermediate representations. This allows large-scale unlabeled data to be useful during training, and also enables transferring learned knowledge to images of unseen object categories, lighting conditions, and shapes. Extensive experiments demonstrate that our method performs well on both intrinsic image decomposition and knowledge transfer.

==> necv/beethoven.tex <==
\begin{figure}[t]   
  %\includegraphics[trim={0 0 0 30pt},clip,width=\linewidth]{fig/pascal.pdf}
  \includegraphics[width=\linewidth]{fig/shader_horizontal.png}
  \vspace{-15pt}
    \caption{Our shading model's outputs after training only on synthetic car models from the ShapeNet dataset \cite{shapenet}. (a) shows the effect of panning the light horizontally and (b) shows the effect of changing the intensity of the light. The input lights are visualized by rendering them onto a sphere. Even though the shader was trained only on synthetic data, it generalizes well to real shapes with no further training. The shape input to (c) is an estimated normals map of a Beethoven bust.}
    \vspace{-15pt}
    \label{fig:beethoven}
\end{figure}

==> necv/macros.tex <==
% require xspace, array

%% layout
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcommand{\xpar}[1]{\noindent\textbf{#1}\ \ }
\newcommand{\vpar}[1]{\vspace{3mm}\noindent\textbf{#1}\ \ }

%% notations
\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\ssect}[1]{\S~\ref{#1}}
\newcommand{\eqn}[1]{Equation~\ref{#1}}
\newcommand{\fig}[1]{Figure~\ref{#1}}
\newcommand{\tbl}[1]{Table~\ref{#1}}

\newcommand{\degree}{\ensuremath{^\circ}\xspace}
\newcommand{\ignorethis}[1]{}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\fcseven}{$\mbox{fc}_7$}

\renewcommand*{\thefootnote}{\fnsymbol{footnote}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\def\naive{na\"{\i}ve\xspace}
\def\Naive{Na\"{\i}ve\xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

%% comments
\definecolor{MyDarkBlue}{rgb}{0,0.08,1}
\definecolor{MyDarkGreen}{rgb}{0.02,0.6,0.02}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{1.0,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}

\newcommand{\tianfan}[1]{\textcolor{MyDarkRed}{[Tianfan: #1]}}
\newcommand{\jw}[1]{\textcolor{MyDarkGreen}{[Jiajun: #1]}}
\newcommand{\katie}[1]{\textcolor{MyDarkBlue}{[Katie: #1]}}
\newcommand{\bill}[1]{\textcolor{MyDarkOrange}{[Bill: #1]}}
\newcommand{\ignore}[1]{}

\def\bR{\mathbb{R}}
\def\cL{\mathcal{L}}
\def\i{^{(i)}}
\def\netname{probabilistic frame predictor\xspace}
\def\Netname{Probabilistic frame predictor\xspace}
\def\gendis{conditional data distribution\xspace}
\def\regdis{variational distribution\xspace}
\def\genmodel{generative model\xspace}
\def\regmodel{recognition model\xspace}
\def\zname{compact motion representation\xspace}

%\newcommand{\myparagraph}[1]{\mbox{}\\[-12mm]\paragraph{#1}}
\newcommand{\myparagraph}[1]{\vspace{-5pt}\paragraph{#1}}


==> necv/model.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.9\linewidth]{fig/schematic.png}
    \vspace{-5pt}
    \caption{RIN contains two convolutional encoder-decoders, one used for predicting the intrinsic images from an input and another for predicting the shading stemming from a light source applied on a shape. The two networks together function as a larger structured autoencoder, forcing a specific type of intermediate representation in order to reconstruct the input image.} %\tianfan{Make the ball slightly larger.}}
    \vspace{-5pt}
    \label{fig:model}
\end{figure}

==> necv/packages.tex <==
% basic
\usepackage{color}%,xcolor}
\usepackage{epsfig}
\usepackage{graphicx}

% figure and table
\usepackage{adjustbox}
\usepackage{array}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float,wrapfig}
\usepackage{hhline}
\usepackage{multirow}
%\usepackage{subcaption}

% font and character
\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{microtype}

% layout
\usepackage{changepage}
\usepackage{extramarks}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{setspace}
\usepackage{soul}
\usepackage{xspace}

% ref
%\usepackage[pagebackref=true,breaklinks=true,colorlinks,citecolor=gray]{hyperref}
%\usepackage[pagebackref=true,breaklinks=true,colorlinks]{hyperref}
% \usepackage{url}

% misc
\usepackage{algorithm, algorithmic}
\usepackage{enumerate}
%\usepackage{todonotes}

==> necv/teaser.tex <==
\begin{figure}[h]
    \vspace{-5pt}
    \centering
    \includegraphics[width=.9\linewidth]{fig/underconstrained_horizontal.png}
    \vspace{-5pt}
    \caption{A porcelain vase (a) along with three predictions (b-d) for its underlying intrinsic images. The set in (c) assumes the contribution from shading is negligible by predicting a completely flat rather than rounded shape. The set in (d) includes the correct shape but assumes red lighting and a much brighter blue color in the regions affected by shading. While the decomposition in (b) is much more inuitively pleasing than either of these alternatives, all of these options are valid in that they combine to exactly form the observed vase. (e) shows a sphere with our visualized normals map as a shape reference.}
    \vspace{-10pt}
    \label{fig:teaser}
\end{figure}

==> packages.tex <==
% basic
\usepackage{color,xcolor}
\usepackage{epsfig}
\usepackage{graphicx}

% figure and table
\usepackage{adjustbox}
\usepackage{array}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float,wrapfig}
\usepackage{hhline}
\usepackage{multirow}
%\usepackage{subcaption} % issues a warning with CVPR/ICCV format

% font and character
\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{microtype}

% layout
\usepackage{changepage}
\usepackage{extramarks}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{setspace}
\usepackage{soul}
\usepackage{xspace}

% ref
\usepackage{url}

% misc
\usepackage{algorithm, algorithmic}
\usepackage{enumerate}
%\usepackage{todonotes} % conflict with CVPR/ICCV format

% Janner
\usepackage{sidecap, wrapfig}


==> text/application.tex <==
\section{Applications}
\label{sec:app}

